Machine Learning with Membership Privacy using Adversarial Regularization

Machine learning models leak information about the datasets on which they are trained. An adversary can build an algorithm to trace the individual members of a model's training dataset. As a fundamental inference attack, he aims to distinguish between data points that were part of the model's training set and any other data points from the same distribution. This is known as the tracing (and also membership inference) attack. In this paper, we focus on such attacks against black-box models, where the adversary can only observe the output of the model, but not its parameters. This is the current setting of machine learning as a service in the Internet. We introduce a privacy mechanism to train machine learning models that provably achieve membership privacy: the model's predictions on its training data are indistinguishable from its predictions on other data points from the same distribution. We design a strategic mechanism where the privacy mechanism anticipates the membership inference attacks. The objective is to train a model such that not only does it have the minimum prediction error (high utility), but also it is the most robust model against its corresponding strongest inference attack (high privacy). We formalize this as a min-max game optimization problem, and design an adversarial training algorithm that minimizes the classification loss of the model as well as the maximum gain of the membership inference attack against it. This strategy, which guarantees membership privacy (as prediction indistinguishability), acts also as a strong regularizer and significantly generalizes the model. We evaluate our privacy mechanism on deep neural networks using different benchmark datasets. We show that our min-max strategy can mitigate the risk of membership inference attacks (close to the random guess) with a negligible cost in terms of the classification error.

==> theory.tex <==
\section{Theoretical results}\label{app:theory}
Our model ultimate goal is to create a classifier function $f$ such that generate similar output distribution for data point from the training data and not training data. We would like algorithm~\ref{alg:training} to converge to such solution.
Our problem setup is similar to the generative adversarial models so we can use similar approach to show correctness of our approach. In this section we use non-parametric functions of $f$ and $h$ for the classifier and attacker respectively. We assume these functions have enough capacity to converge to the optimal probability density function. We use $p_{f(D)}$ and $p_{f(D')}$ to show the distribution of the outputs of network $f$ for the data instances in $D$ and $D'$ respectively.

\paragraphb{Optimal Attacker:}
For any fixed given classifier $f$ the best attacker $h$ is:
\begin{align*}
h*_(f)(f(x))= \frac{P_{f(D)}(f(x))}{P_{f(D)}(f(x))+P_{f(D')}(f(x))}
\end{align*}
\paragraphb{Proof:} Attacker wants to maximize equation~\eqref{eq:gain}, so we have:
\begin{align}
	\Gain_f(h) = 
	&\expected{\log( h(x, y, f(x)))}{(x,y) \sim \set{D}} + 
	\expected{\log(1 - h(x, y, f(x)))}{(x,y) \sim \prob(\rv{X}, \rv{Y})} \\
	\Gain_f(h) =& \int_{x,y} p_{D}(x,y) p_{f(D)}(f(x)) \log( h(x, y, f(x))) \\
	&+  \int_{x',y'} p_{D'}(x',y') p_{f(D')}(f(x')) \log( 1-h(x, y, f(x)))
\end{align}
Since distribution of data in $D$  and $D'$ are similar we can rewrite as follow:
 \begin{align}
	\Gain_f(h) =& \int_{x,y}  p_{f(D)}(f(x)) \log( h(x, y, f(x))) \\
	&+  \int_{x',y'} p_{f(D')}(f(x')) \log( 1-h(x, y, f(x)))
\end{align}
Maximum values of this function~\cite{goodfellow2014generative} happens when $h(x)$ is:
\begin{align}
h_(f)(f(x))= \frac{P_{f(D)}(f(x))}{P_{f(D)}(f(x))+P_{f(D')}(f(x))}
\end{align}
\lemma{Optimal game classifier:}
Function $f^*$ among all of classification functions which can get a fixed specific value of classification loss (i.e. equation ~\eqref{eq:closs_emp}), is global minimization function if and only if $p_{f^*(D)}=p_{f^*(D')}$.
\proof 
When the value of classification loss is fixed, game will reduce to 
\begin{align}
&\min\limits_f\max\limits_h   \expected{\log(h(x, y, f(x)))}{(x,y) \sim \set{D}} + 
	\expected{\log(1 - h(x, y, f(x)))}{(x,y) \sim \prob(\rv{X}, \rv{Y})}
\end{align}
So we can use theorem 1 in~\cite{goodfellow2014generative} proves $f^*$ global minimization function if and only if $p_{f^*(D)}=p_{f^*(D')}$.

\par We showed the best strategy for the classifier is to create similar output probability for the data instances in the training set and data points out side of training set. Also Proposition 2 in ~\cite{goodfellow2014generative} shows that a gradient descent algorithm can eventually converge.
